High Frequency Residual Learning for Multi-Scale Image Classification

We present a novel high frequency residual learning framework, which leads to a highly efficient multi-scale network (MSNet) architecture for mobile and embedded vision problems. The architecture utilizes two networks: a low resolution network to efficiently approximate low frequency components and a high resolution network to learn high frequency residuals by reusing the upsampled low resolution features. With a classifier calibration module, MSNet can dynamically allocate computation resources during inference to achieve a better speed and accuracy trade-off. We evaluate our methods on the challenging ImageNet-1k dataset and observe consistent improvements over different base networks. On ResNet-18 and MobileNet with alpha=1.0, MSNet gains 1.5% accuracy over both architectures without increasing computations. On the more efficient MobileNet with alpha=0.25, our method gains 3.8% accuracy with the same amount of computations.

==> sections/discussion.tex <==
\section{Discussion}

\subsection{Generalization to Other Networks}
Unlike MSDNet \cite{huang2017densely} that requires dense connections to avoid the problem that classifiers at early stages will hamper the training of classifier at later stages, our method can be easily generalized to any existing network architectures.

If we denote a group of features having the same resolution as a ``stage'' (e.g. most networks like ResNet have 5 stages with resolutions 1/2, 1/4, 1/8, 1/16, 1/32 of the input resolution), our method is to upsample the features at the end of each stage (stage-end features) of LRN and add the upsampled features to the the corresponding stage-end features at HRN. The new features are passed to the next stage in HRN.

Due to limited resources, we only demonstrate our method on three networks. But the effectiveness of method on a large range of networks (ResNet is a classical network, MobileNet is a mobile-level network and DenseNet is a network with state-of-the-art performance). 

\subsection{Future Works}
\subsubsection{Generalization to other tasks}
An interesting question is that can this idea of reusing low resolution feature be applied to other tasks? We think the answer is YES. For example, we can generalize this idea to object detection. The key challenge in detection is how to obtain multi-scale features using the same depth of network but without significant increase of the input image resolution and computation. Our proposed network has a potential to generate multi-scale feature maps that can be end-to-end pretrained. But we admit there is still much work to do to verify the idea for detection.

\subsubsection{Generalization to more scales}
Throughout our experiments, we only use two scales in our network. An interesting research direction is to add more scales in our network. However, one needs to handle the following two problems when adding more resolutions:
\begin{enumerate}
\item When adding a lower resolution (\eg adding a $56\times56$ resolution to our currently used 112/224 pair), the resolution of the feature map may be too small to contain any useful information.
\item When adding a higher resolution (\eg adding a $448\times448$ resolution to our currently used 112/224 pair), the introduced computation on the 448 resolution may be too large to achieve better speed-accuracy trade-off.
\end{enumerate}
One suggesting is to add a ``decimal resolution'' which is not a factor of 2 to the original $224\times224$ resolution.
